Resume-ing Control: (Mis)Perceptions of Agency Around GenAI Use in Recruiting Workflows

When generative AI (genAI) systems are used in high-stakes decision-making, its recommended role is to aid, rather than replace, human decision-making. However, there is little empirical exploration of how professionals making high-stakes decisions, such as those related to employment, perceive their agency and level of control when working with genAI systems. Through interviews with 22 recruiting professionals, we investigate how genAI subtly influences control over everyday workflows and even individual hiring decisions. Our findings highlight a pressing conflict: while recruiters believe they have final authority across the recruiting pipeline, genAI has become an invisible architect that shapes the foundational building blocks of information used for evaluation, from defining a job to determining good interview performances. The decision of whether or not to adopt was also often outside recruiters' control, with many feeling compelled to adopt genAI due to calls to integrate AI from higher-ups in their business, to combat applicant use of AI, and the individual need to boost productivity. Despite a seemingly seismic shift in how recruiting happens, participants only reported marginal efficiency gains. Such gains came at the high cost of recruiter deskilling, a trend that jeopardizes the meaningful oversight of decision-making. We conclude by discussing the implications of such findings for responsible and perceptible genAI use in hiring contexts.

==> tab-figs/codebook.tex <==
\begin{table*}[]
\tiny
\begin{tabularx}{\linewidth}{|X|X|}
\hline
\textbf{Agency-focused} & \textbf{Candidate-focused} \\ \hline
{\begin{tabularx}{\linewidth}[c]{@{}X@{}}
\textit{Auto/AI-Resistant Work}: Assertion that a specific task cannot be performed by AI\\ 
\textit{Deference to AI}: Instance where the participant trusts AI\\ 
\textit{Employer AI Red Line}: Determination of when AI should not be used in the recruitment process\\ 
\textit{Human Agency Maintained}: Belief that the participant maintains decision-making agency\\ 
\textit{Lack of Trust in AI/Skepticism}: Skepticism toward the use of AI in general or a specific task\\ 
\textit{Shared Decision-making}: Belief that AI has some impact on the decision-making process\\ 
\textit{Perceived Human Manual}: Claim that participant is manually performing a certain task\end{tabularx}} & {\begin{tabularx}{\linewidth}[c]{@{}X@{}}
\textit{Candidate use of AI}: How candidates use AI\\ 
\textit{Candidate effort stands out}: The manual effort of a candidate is obvious when reviewing their application\\ 
\textit{Desired candidate skillsets}: The skills that the participant is looking for\\ 
\textit{Applicant-recruiter arms race}: Participant's use of AI to combat candidate's use\\ 
\textit{Fake candidates}: Discussion of reportedly ``fake'' candidates\\ 
\textit{High volume of applications}: Capturing the great demand on recruiters for reviewing applications\end{tabularx}} \\ \hline
\textbf{Company-focused} & \textbf{Impacts/future}  \\ \hline
{\begin{tabularx}{\linewidth}[c]{@{}X@{}}
\textit{Business culture}: What is the company's culture like?\\ 
\textit{Business size}: How large is the company\\
\textit{Pressure to use AI in business}: Participant reporting pressure to use AI from their employer\\ 
\textit{Stage of AI adoption}: How much AI the employer is incorporating company-wide\\ 
\textit{Prohibitive cost of AI}: Statement that AI tools are out of the price range for a participant's company\end{tabularx}} 
& {\begin{tabularx}{\linewidth}[c]{@{}X@{}}
\textit{AI Future Potential}: Looking forward to AI's future impact\\ 
\textit{Legal and Privacy Risk}: Reported fear of risk or performing actions that constitute risk\\ 
\textit{Loss of Skill/Deskilling}: Observed behavior that reflects deskilling\\ 
\textit{Overpromising of AI}: Belief that AI marketing has overpromised on the utility of AI\\ 
\textit{AI Used Differently by Generations}: Pattern that different age groups use AI in disparate manners\\ 
\textit{Two-tiered AI use}: Different usage of AI depending on qualities of the role or candidate\end{tabularx}}\\ \hline
\textbf{Participant/role information} & \textbf{Performance of AI systems}\\ \hline
{\begin{tabularx}{\linewidth}[c]{@{}X@{}}
\textit{Job Level Type}: The level of position that the participant hires for\\ 
\textit{Participant Background}: Information about participant's role and experience\\ 
\textit{Self-Assessment of AI Proficiency}: A participant's confidence in their use of AI\\ 
\textit{Time in Role}: How long has the participant been in this role\end{tabularx}} 
& {\begin{tabularx}{\linewidth}[c]{@{}X@{}}AI evaluates candidates badly: Inconsistent or incorrect evaluation of candidates\\ 
\textit{AI is biased}: Relaying of concerns about biased outputs from AI systems\\ 
\textit{AI lacks nuance}: Discusses that AI systems may be brittle or do not understand humans\\ 
\textit{AI makes More More Work}: Claim that the participant's use of AI increases their workload\\ 
\textit{AI Reveals Overlooked Details}: AI provides the participant with a more detailed interpretation of the input\\ 
AI Saves Time: The use of AI reduces time spent on a task\\ 
\textit{AI Tool Performance}: Reflects how well the AI tool is seen to perform in general\\ 
\textit{AI Use is Essential for Efficiency}: Belief that one's use of AI is essential for the efficient completion of tasks\end{tabularx}}                                                                            \\ \hline
\textbf{Recruitment stage}                                             & \textbf{Task Type} \\ \hline
{\begin{tabularx}{\linewidth}[c]{@{}X@{}}
\textit{Assessment}: Process of forming a judgment on a candidate\\ \textit{Conceptualizing/Themeing}: Generation of a job description\\ \textit{Final Decision-making}: Selection of candidate(s) to send an offer to\\ 
\textit{Interviewing}: Conversations with candidates\\ 
\textit{Logistics}: Planning interviews, sending communication, etc.\\ 
\textit{Sourcing}: Finding candidates to apply to a job opening\\ 
\textit{Screening}: Comparing a candidate's skills and qualifications to the job requirements\end{tabularx}}                                                                                                                                                            & {\begin{tabularx}{\linewidth}[c]{@{}X@{}}
\textit{Agentic AI}: Using AI agents to complete a task\\ 
\textit{AI Content Generation}: Using generative AI to produce communication, summaries, etc.\\ 
\textit{Analogue-Technical Processes}: A process combining both technical and manual methods\\ 
\textit{Grouping}: Classifying candidates in a fixed number of groups\\ 
\textit{Keyword Searching}: Looking for specific keywords in a document (e.g. resume)\\ 
\textit{Manual Work}: Lack of reliance on recruitment-specific tools in a task\\ 
\textit{Transcription}: Translation from a recording to text\\ 
\textit{Summarizing}: Reduction of an input into a shortened form\\ 
\textit{Ranking}: Comparing candidates to one another individually\\ 
\textit{Research/Information Gathering}: Process of learning about a certain domain\\ 
\textit{System Indicators of Job Compatibility}: How is job compatibility reflected to the participant\end{tabularx}} \\ \hline
\end{tabularx}
\end{table*}

==> tab-figs/taxonomy-groups.tex <==
\begin{table*}
\centering
\caption{\todo{Something about the table}}
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\linewidth}{|
p{0.31\linewidth}
|X|X|X|X|}
\hline
 & \textit{\textbf{\begin{tabular}[l]{@{}l@{}}Conceptual-\\ izing\end{tabular}}}
 & \textit{\textbf{Sourcing}}
 & \textit{\textbf{Screening}}
 &\textit{\textbf{Interviewing}} \\

 & Development of a new job posting
 & Actively searching for new candidates
 & Reviewing applicants who have applied
 & Verbally communicating with current applicants \\
\hline
\textit{\textbf{Summarizing}}

Reducing an input into a brief overview
 & \multicolumn{2}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 & Candidate summary
 & Interview summary \\
\hline
\textit{\textbf{Generating}}

Generating an output based on a prompt
 & Job description 
 
 generation
 & \multicolumn{2}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 & Interview question generation \\
\hline
\textit{\textbf{Leading Discussion}}

An AI system autonomously leading communication with a candidate
 & \multicolumn{2}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 & AI-led screening
 & AI-led 
 
 interview \\
\hline
\textit{\textbf{Transcribing}}

The production of a transcript from a recorded call
 & \multicolumn{3}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 & Interview transcription \\
\hline
\textit{\textbf{Filtering}}

Reducing a certain number of candidates to a smaller number based on filters
 & \multicolumn{1}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 & Database 
 
 filtering
 & Candidate filtering
 & \cellcolor{lightgray} \\
\hline
\textit{\textbf{Grouping}}

Classifying candidates in a fixed number of groups
 & \multicolumn{2}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 & Qualification grouping, Candidate fraud detection
 &  \cellcolor{lightgray}\\
\hline
\textit{\textbf{Ranking}}

Comparing candidates to one another individually
 & \multicolumn{2}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 & Match ranking / scores
 &  \cellcolor{lightgray}\\
\hline
\textit{\textbf{Individual Evaluation}}

Individually determining one’s performance or fitness given certain criteria
 & \multicolumn{3}{c|}{\cellcolor{lightgray}} 
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 %& \cellcolor{gray}
 & Interview scoring, Interviewer feedback \\
\hline

\textit{\textbf{Full/Partial Automation}}

Automating single or multiple stages of the recruitment pipeline
 & \multicolumn{4}{c|}{Covers all or part of the pipeline}\\
 \hline
\end{tabularx}
\end{table*}

